On Testing of Samplers

Given a set of items $\mathcal{F}$ and a weight function $\mathtt{wt}: \mathcal{F} \mapsto (0,1)$, the problem of sampling seeks to sample an item proportional to its weight. Sampling is a fundamental problem in machine learning. The daunting computational complexity of sampling with formal guarantees leads designers to propose heuristics-based techniques for which no rigorous theoretical analysis exists to quantify the quality of generated distributions. This poses a challenge in designing a testing methodology to test whether a sampler under test generates samples according to a given distribution. Only recently, Chakraborty and Meel (2019) designed the first scalable verifier, called Barbarik1, for samplers in the special case when the weight function $\mathtt{wt}$ is constant, that is, when the sampler is supposed to sample uniformly from $\mathcal{F}$ . The techniques in Barbarik1, however, fail to handle general weight functions. The primary contribution of this paper is an affirmative answer to the above challenge: motivated by Barbarik1 but using different techniques and analysis, we design Barbarik2 an algorithm to test whether the distribution generated by a sampler is $\varepsilon$-close or $\eta$-far from any target distribution. In contrast to black-box sampling techniques that require a number of samples proportional to $|\mathcal{F}|$ , Barbarik2 requires only $\tilde{O}(tilt(\mathtt{wt},\varphi)^2/\eta(\eta - 6\varepsilon)^3)$ samples, where the $tilt$ is the maximum ratio of weights of two satisfying assignments. Barbarik2 can handle any arbitrary weight function. We present a prototype implementation of Barbarik2 and use it to test three state-of-the-art samplers.

==> bibliography.tex <==
%
% ---- Bibliography ----
%
% BibTeX users should specify bibliography style 'splncs04'.
% References will then be sorted and formatted in the correct style.
%
 \bibliographystyle{splncs04}
 \bibliography{Report}
%
%\begin{thebibliography}{8}
%\bibitem{ref_article1}
%Author, F.: Article title. Journal \textbf{2}(5), 99--110 (2016)
%
%\bibitem{ref_lncs1}
%Author, F., Author, S.: Title of a proceedings paper. In: Editor,
%F., Editor, S. (eds.) CONFERENCE 2016, LNCS, vol. 9999, pp. 1--13.
%Springer, Heidelberg (2016). \doi{10.10007/1234567890}
%
%\bibitem{ref_book1}
%Author, F., Author, S., Author, T.: Book title. 2nd edn. Publisher,
%Location (1999)
%
%\bibitem{ref_proc1}
%Author, A.-B.: Contribution title. In: 9th International Proceedings
%on Proceedings, pp. 1--2. Publisher, Location (2010)
%
%\bibitem{ref_url1}
%LNCS Homepage, \url{http://www.springer.com/lncs}. Last accessed 4
%Oct 2017
%\end{thebibliography}

==> prelims.tex <==
\section{Notations and Preliminaries}\label{sec:prelims}
A Boolean variable is denoted by a lowercase letter. A Boolean formula $\varphi$ is a function, $\varphi: \{0,1\}^* \rightarrow \{0,1\}$.
 For a Boolean formula $\varphi$, the set of variables appearing in $\varphi$, called the \textit{support} of $\varphi$, is denoted by $Supp(\varphi)$.
An assignment $\sigma \in \{0,1\}^{|Supp(\varphi)|}$ to the variables of $\varphi$ is a \textit{satisfying assignment} or \textit{witness}  if it makes $\varphi$  evaluate to $1$. We denote the set of all satisfying assignments of $\varphi$ as $R_{\varphi}$. For $S\subseteq Supp(\varphi)$, we use $\sigma_{\downarrow{S}}$ to indicate the projection of $\sigma$ over the set of variables in $S$. And we denote by $R_{\varphi_{\downarrow{S}}}$ the set $\{\sigma_{\downarrow{S}}\ |\ \sigma\in R_{\varphi}\}$.

  \begin{definition}[Weight Function]
 	For a set $S$ of Boolean variables, a weight function $\mathtt{wt}: \{0,1\}^{|S|} \rightarrow (0,1)$ maps each assignment to some weight.
 \end{definition}

\begin{definition}[Sampler]
A sampler $\mathcal{G}(\varphi, S, \mathtt{wt}, \tau)$ is a randomized algorithm that takes in a Boolean formula $\varphi$, a weight function $\mathtt{wt}$, a set $S\subseteq Supp(\varphi)$ and a positive integer $\tau$ and outputs $\tau$  independent samples from $R_{\varphi_{\downarrow {S}}}$.  For brevity of notation we may sometimes refer to a sampler as $\mathcal{G}(\varphi, \tau)$ or $\mathcal{G}(\varphi)$ or just $\mathcal{G}$.

For any $\sigma \in \{0,1\}^{|S|}$ the probability of the sampler outputting $\sigma$ is denoted by $p_\mathcal{G}(\varphi, S, \sigma)$ (or $p_{\mathcal{G}}(\varphi, \sigma)$ when the set $S$ in question is clear from the context). Or in other words,
\begin{align*}
    p_\mathcal{G}(\varphi,S, \sigma) = \Pr \left[\mathcal{G}(\varphi, S) \mbox{ returns } \sigma \right]
\end{align*}
\end{definition}
We use $D_{\mathcal{G}(\varphi, S)}$  to represent the distribution induced by $\mathcal{G}(\varphi,S)$ on $R_{\varphi_{\downarrow{S}}}$. When the set $S$ is understood from the context we will denote $D_{\mathcal{G}(\varphi, S)}$ by $D_{\mathcal{G}(\varphi)}$.

\begin{definition}[Ideal Sampler]\label{def:ideal_weighted}
For a weight function $\mathtt{wt}$, a sampler $\mathcal{A}(\varphi ,S, \tau)$ is called an ideal sampler w.r.t. weight function $\mathtt{wt}$ if for all $\sigma \in R_{\varphi_{\downarrow{S}}}$:
	\begin{align*}
	p_\mathcal{A}(\varphi,S, \mathtt{wt}, \sigma) = \frac{\wt{\sigma} }{\sum_{\sigma'\in R_{\varphi_{\downarrow{S}}}}\wt{\sigma'}}
	\end{align*}
In the rest of the paper, $\mathcal{A}(\cdot,\cdot,\cdot, \cdot)$  denotes the ideal sampler. Similar to $\mathcal{G}$, we will often refer to the ideal sampler with $\mathcal{A}$ when other parameters are clear from the context. 
%In the interests of readability we will omit the $\mathtt{wt}$ superscript whenever the weight function is obvious from the context.
\end{definition}
When the sampler samples according to the uniform distribution it is called a uniform sampler.  In that case the weight function becomes $\mathtt{wt}(\sigma) = \frac{1}{|R_{\varphi}|}$.

\begin{definition}[tilt]\label{defn:tilt}
    For any Boolean formula $\varphi$, and weight function $\mathtt{wt}$, we define a function $tilt$:
    \begin{align*}
        tilt(\mathtt{wt},\varphi) = 
%        \frac{\underset{\sigma_1 \in R_\varphi}{\max}\; {\mathtt{wt}}(\sigma_1)}{\underset{\sigma_2 \in R_\varphi}{\min}\; {\mathtt{wt}}(\sigma_2)} = 
                 \underset{\sigma_1,\sigma_2 \in R_\varphi}{\max}\;\frac{\mathtt{wt}(\sigma_1)}{\mathtt{wt}( \sigma_2)}.
%        =\underset{\sigma_1,\sigma_2 \in R_\varphi}{\max}\;\frac{ p_\mathcal{A}(\varphi,\sigma_1)}{ p_\mathcal{A}(\varphi,\sigma_2)}
    \end{align*}

\end{definition}
Our goal is to design a program that can test the quality of a sampler with respect to an ideal sampler. In this regard, we have to define the concept of the distance of the sampler from the ideal sampler.
We use two different notions of distance.

\begin{definition}[$\varepsilon$-closeness and $\eta$-farness]\label{def:closeness_and_farness}
A sampler $\mathcal{G}$ is $\varepsilon$-additive-close (or simply $\varepsilon$-close) to an ideal sampler $\mathcal{A}$, if for all $\varphi$ and  all  $\sigma \in R_{\varphi}$, the following holds:
 \begin{align*}
 (1-\varepsilon)p_\mathcal{A}(\varphi,\sigma)\leq p_\mathcal{G}(\varphi,\sigma) \leq (1+\varepsilon)p_\mathcal{A}(\varphi,\sigma)
\end{align*}
For a formula $\varphi$, a sampler $\mathcal{G}(\varphi)$ is $\eta$-$\ell_1$-far (or simply $\eta$-far) from the ideal sampler $\mathcal{A}(\varphi)$, if
\begin{align*}
   \sum_{\sigma \in R_{\varphi}} |p_\mathcal{A}(\varphi, \sigma) - p_\mathcal{G}( \varphi, \sigma) | \geq \eta
\end{align*}
\end{definition}


\begin{definition}[$(\varepsilon,\eta, \delta)$-tester for samplers]
A $(\varepsilon, \eta, \delta)$-tester for samplers is a randomized algorithm that takes a sampler $\mathcal{G}$, an ideal sampler $\mathcal{A}$, a tolerance parameter $\varepsilon$, an intolerance parameter $\eta$, a guarantee parameter $\delta$ and a CNF formula $\varphi$ and returns {\accept} or {\reject} with the following guarantees:
\begin{itemize}
	\item If $\mathcal{G}$ is  $\varepsilon$-close to $\mathcal{A}(\varphi)$,  then the tester returns {\accept} with probability at least $(1-\delta)$.
	\item If $\mathcal{G}(\varphi)$ is $\eta$-far from $\mathcal{A}(\varphi)$ then the tester returns {\reject} with probability at least $(1-\delta)$.
\end{itemize}
\end{definition}




%\subsection{Chain Formula}\todo{Add description about chain formulas in the Appendix}

%A crucial component that we use in our algorithm is that of chain formulas. Chain formulas, introduced in \cite{CFMV15}, are a special class of Boolean formulas. 
%Given a positive integer $k$ and $m$, chain formulas provide an efficient construction of a Boolean formula $\psi_{k,m}$ with exactly $k$ satisfying assignments with $\ceil{log(k)} \leq m$ variables.
%The chain formula encoding is useful to us in two ways:
%(1) It lets us simulate weighted sampling with a uniform sampler (2) We can generate formulas with a specified number of satisfying assignments.


\subsection{Chain Formula, Kernel and Non-Adversarial Assumption}

A crucial subroutine that we use in our algorithm helps us to draw ``conditional samples" from $R_{\varphi_{\downarrow {S}}}$. This is similar to the subroutine {\kernel} used by the {\oldbarbarik} in \cite{CM19}. By an abuse of notation we will also use {\kernel} 
to describe a collection of functions. 

\begin{definition}
	{\kernel}  takes in a Boolean formula $\varphi$, $S \subseteq Supp(\varphi)$, and two assignments $\sigma_1, \sigma_2 \in R_{\varphi \downarrow S}$,  and returns $\hat{\varphi}$ such that $R_{\hat{\varphi}\downarrow{S}} = \{\sigma_1, \sigma_2 \}$. 
\end{definition}
%\todo{Add description about the similarity with respect to barbarik}

In  \cite{CM19} it was proved that if a sampler, that is far from uniform,  satisfied a ``non-adversarial condition" then the tester {\oldbarbarik} would reject such a sampler. And it was assumed in \cite{CM19} that many samplers that are in use would in fact satisfy the 
``non-adversarial condition" and the success of {\oldbarbarik} kind of validated the assumption.  The ``non-adversarial condition" can be best described using the following definition.

\begin{definition}\label{def:nonadversarial} 
	A sampler $\mathcal{G}$ is non-adversarial w.r.t.  a particular {\kernel} for $\varphi$ if for all $S \subseteq Supp(\varphi)$, $  \sigma_1, \sigma_2 \in  R_{\varphi_{\downarrow {S}}}$, let   $\hat{\varphi} \gets \kernel(\varphi, S, \sigma_1, \sigma_2)$ then
	the output of $\mathcal{G}(\hat{\varphi}, \mathtt{wt}, S, \tau)$ is $\tau$ independent samples from the conditional distribution $\mathcal{D}_{\mathcal{G}(\varphi) \downarrow{T}}$, where $T=\{\sigma_1, \sigma_2\}$.
\end{definition}

For proving the correctness of our tester against a particular sampler we will using the above definition, similar to its usage in \cite{CM19}.  While we don't have a fool-proof of technique ensure that a sampler is  non-adversarial w.r.t.  a particular {\kernel} 
we believe that a {\kernel} with certain other properties would work for most samplers that are now in use. To design such a {\kernel} we crucially use chain formulas. A description if chain formulas is given in the Appendix. \todo{Relate it to experiments}




